Are All Losses Created Equal: A Neural Collapse Perspective

While cross entropy (CE) is the most commonly used loss to train deep neural networks for classification tasks, many alternative losses have been developed to obtain better empirical performance. Among them, which one is the best to use is still a mystery, because there seem to be multiple factors affecting the answer, such as properties of the dataset, the choice of network architecture, and so on. This paper studies the choice of loss function by examining the last-layer features of deep networks, drawing inspiration from a recent line work showing that the global optimal solution of CE and mean-square-error (MSE) losses exhibits a Neural Collapse phenomenon. That is, for sufficiently large networks trained until convergence, (i) all features of the same class collapse to the corresponding class mean and (ii) the means associated with different classes are in a configuration where their pairwise distances are all equal and maximized. We extend such results and show through global solution and landscape analyses that a broad family of loss functions including commonly used label smoothing (LS) and focal loss (FL) exhibits Neural Collapse. Hence, all relevant losses(i.e., CE, LS, FL, MSE) produce equivalent features on training data. Based on the unconstrained feature model assumption, we provide either the global landscape analysis for LS loss or the local landscape analysis for FL loss and show that the (only!) global minimizers are neural collapse solutions, while all other critical points are strict saddles whose Hessian exhibit negative curvature directions either in the global scope for LS loss or in the local scope for FL loss near the optimal solution. The experiments further show that Neural Collapse features obtained from all relevant losses lead to largely identical performance on test data as well, provided that the network is sufficiently large and trained until convergence.

==> NeurIPS_2022/Sections/main_results.tex <==

%In next section, we will analyze the optimization landscape for the objective function in \eqref{eq:obj}.

In this section, we present our study on global optimality conditions as well as the optimization landscape of the nonconvex loss in \eqref{eq:obj}.
%\zz{Since each subsection only contains one result, do we still need to put them as subsections?}


%To ease the presentation, throughout the paper, denote by $\vw_k$ as the $k$-th row of $\mW$, i.e., $\mW = \begin{bmatrix}\vw_1 & \cdots & \vw_K \end{bmatrix}^\top$.

\begin{comment}
\subsection{Global Optimality Conditions for \eqref{eq:obj}}
We begin by characterizing the global solutions of \eqref{eq:obj}, showing that the Simplex ETFs are its only global minimizers. 
\end{comment}

% in the following result.
%First of all, we can show that the Simplex ETF are the only global solutions. 
\begin{theorem}[Global Optimality Conditions]\label{thm:global-minima}
	Assume that the feature dimension $d$ is no smaller than the number of classes $K$, i.e. $d\ge \revise{K-1}$, and the number of training samples in each class is balanced, $n = n_1 = \cdots = n_K$. Then any global minimizer $(\mW^\star, \mH^\star,\vb^\star)$ of $f$ in \eqref{eq:obj} satisfies 
\begin{align}
\begin{split}
        &  w^\star  :\;=\; \norm{\mb w^{\star 1}}{2} \;=\; \norm{\mb w^{\star 2} }{2} \;=\; \cdots \;=\; \norm{\mb w^{\star K} }{2} , \quad \text{and}\quad \mb b^\star = b^\star \mb 1, \\ 
    & \vh_{k,i}^\star \;=\;  \sqrt{ \frac{ \lambda_{\mb W}  }{ \lambda_{\mb H} n } } \vw^{\star k},\quad \forall \; k\in[K],\; i\in[n],  \quad \text{and} \quad  \ol{\mb h}_{i}^\star \;:=\; \frac{1}{K} \sum_{j=1}^K \mb h_{j,i}^\star \;=\; \mb 0, \quad \forall \; i \in [n],
\end{split}
\end{align}
\vspace{-0.2in}

where either $b^\star = 0$ or $\lambdab=0$, and the matrix $\mW^{\star\top} \in \bb R^{d \times K} $ forms a $K$-Simplex ETF (defined in Definition \ref{def:simplex-ETF}) up to some scaling, in the sense that  the normalized matrix $\mb M := \frac{1}{w^\star} \mW^{\star\top} $ satisfies
\begin{align}\label{eqn:simplex-ETF-closeness}
    \mb M^\top \mb M \;=\; \frac{K}{K-1}  \paren{ \mb I_K - \frac{1}{K} \mb 1_K \mb 1_K^\top }.
\end{align}

\end{theorem}
%\zz{Here $\mb M \mb M^\top \;=\; \mb M^\top \mb M$ is not true. We only have $\bm M^\top \bm M = \frac{K}{K-1}  \paren{ \mb I_K - \frac{1}{K} \mb 1_K \mb 1_K^\top }$.}

% \cy{This seems to be suggesting that feature dimension $d$ should not affect the performance of the model once we have $d > K$. This is a bit contradicting with the belief that wider networks are better. Maybe we can do some experiments with varying $d$ and see if the acc curve is mostly flat with $d > K$ and drops quickly with $d < K$. Also interesting is that it requires $d > K$ but I wonder if there can be any comment for the case $d = K$.}

% \zz{Good point. \Cref{thm:global-minima} actually works when $d=K$, but \Cref{thm:global-geometry} requires $d> K$.}

% \cy{Thanks, maybe better to say $d \ge K$ in \Cref{thm:global-minima} since there is a discussion of the case $d = K$ for \Cref{thm:global-geometry}? Also maybe better to say $d \ge K$ is ``tight'' (see below)} \zz{Agree. I have uncolored the sentence. Thanks.}

At a high level, our proof (in Appendix \ref{app:thm-global}) finds lower bounds for the loss in \eqref{eq:obj} and studies the conditions for the lower bounds to be achieved, similar to \cite{lu2020neural,fang2021layer}.  As can be seen in this result, any global solution of the loss function \eqref{eq:obj} exhibits \NC\;in the sense that the variability of output features $\{\vh_{k,i}^\star\}_{i=1}^n$ of each class $k$ ($1\leq k\leq K$) collapses to zero, and any pair of features $( \vh_{k_1,i}^\star, \vh_{k_2,j}^\star )$ from different classes $k_1\not = k_2$ are maximally separated. %under the constraint of equal-sized angles between all classes. 
Similar results have been obtained in \cite{fang2021layer,lu2020neural,weinan2020emergence}, which considered different problem formulations, as we have discussed in \Cref{sec:layer-peeled-model}.

\vspace{-.05in}
\begin{itemize}[leftmargin=*]
    \item \textbf{Relationship between Class Number $K$ and Feature Dimension $d$.} The requirement that $d \ge \revise{K-1}$ is necessary for  \Cref{thm:global-minima} to hold, simply because $K$ vectors in $\bb R^d$ cannot form a $K$-Simplex ETF if $K>\revise{d+1}$. However, the relationship $d \ge K$ is often true in practice. In general, and in overparameterized models in particular, the feature dimension, $d$, is significantly larger than the number of classes, $K$. For example, the dimension of the features of a ResNet \cite{he2016deep} is typically set to $d=512$ for CIFAR10 \cite{krizhevsky2009learning}, a dataset with $K = 10$ classes. This dimension grows to $d=2048$ for ImageNet \cite{deng2009imagenet}, a dataset with $K = 1000$ classes.
    \item \textbf{Interpretations on the Bias Term $\mb b^\star$.} In contrast to previous works \cite{fang2021layer,lu2020neural,weinan2020emergence}, we consider the bias term in the unconstrained feature model \eqref{eq:obj}. Our result indicates that a collapsing phenomenon also exists in the bias term $\vb^\star$, in the sense that all the elements of $\vb^\star$ are identical. When the features $\mb H$ are completely unconstrained, our result implies that removing the bias term $\vb$ has no influence on the performance of the classifier. However, it should be noted that the ReLU unit is often applied at the end of the penultimate layer, so that $\mb H$ should be constrained to be nonnegative, $\mb H \geq \mb 0$. In such cases, $\overline \vh_i^\star$ will no longer be zero, and neither will $\mb b^\star$. Here, the bias term $\mb b^\star$ will compensate for the global mean of the features, so that the globally-centered features still form a Simplex ETF \cite{papyan2020prevalence}.\footnote{Suppose that an optimal solution to \eqref{eq:obj} is $(\mW^\star,\mH^\star,\vb^\star)$, satisfying the conditions in \Cref{thm:global-minima}. There exists a nonzero vector $\mb \alpha \in \bb R^d$ such that $\widetilde \mH^\star = \mH^\star + \valpha \mb 1^\top \ge 0$. Here, $\valpha \mb $ can be viewed as the global mean of $\widetilde \mH^\star$ since $\mH^\star$ has mean zero. Then, let $\widetilde\vb^\star = - \mb W^\star \valpha$, so that $\wt{\mb W}^\star \widetilde \mH^\star + \widetilde\vb^\star \mb 1^\top \;=\; \mb W^\star \mH^\star + (\mb W^\star \valpha + \widetilde\vb^\star)\mb 1^\top \;=\; \mW^\star\mH^\star$. Therefore, we can see that $(\wt{\mW}^\star,\widetilde\mH^\star,\widetilde\vb^\star)$ achieves the same cross-entropy loss as $(\mW^\star,\mH^\star,\vb^\star)$. } %\js{i think it might be worthwhile to show this formally as a corollary. Otherwise people who don't read the footnote in detail might think "oh, their result doesn't apply to the case of nonnegative features".} \zz{Good point. This is what we did before, but then we realized we can't formally prove it because of the weight decay. Thus, we add a footnote and show the case for cross-entropy.}
    %in the nonnegative orthant. 
\end{itemize}

\begin{comment}
Moreover, we can show the following when $\mb H \geq \mb 0$.
\begin{corollary}[Global Optimality under the Nonnegativity Constraint $\mb H\geq \mb 0$]
Suppose that an optimal solution to \eqref{eq:obj} \zz{with $\lambdab = 0$.} is $(\mW^\star,\mH^\star,\vb^\star)$, satisfying the conditions in \Cref{thm:global-minima}. Then $(\wt{\mW}^\star,\wt{\mH}^\star,\wt{\vb}^\star)$, with $\wt{\mW}^\star = \mb W^\star$, $\wt{\mH}^\star =  \mH^\star + \valpha \mb 1^\top$, and $\wt{\mb b}^\star = - \mb W^\star \valpha$, forms a global solution to 
\begin{align*}
     \min_{\mb W , \mb H,\mb b  } \; f(\mb W,\mb H,\mb b) , \quad \text{s.t.}\quad \mb H \;\geq\; \mb 0,
\end{align*}
where $\mb \alpha \in \bb R^d$ is some nonzero vector chosen such that $\widetilde \mH^\star = \mH^\star + \valpha \mb 1^\top \ge 0$.
\end{corollary}
Therefore, by subtracting a global mean $\valpha \mb 1^\top$ from $\widetilde \mH^\star$, the dual pair $(\wt{\mW}^\star, \wt{\mH}^\star - \valpha \mb 1^\top)$ are still Simplex ETFs.

\begin{proof}
Here, $\valpha \mb 1^\top$ can be viewed as the global mean of $\widetilde \mH^\star$ since $\mH^\star$ has mean zero. Then, let $\widetilde\vb^\star = - \mb W^\star \valpha$, so that 
\begin{align*}
    \wt{\mb W}^\star \widetilde \mH^\star + \widetilde\vb^\star \mb 1^\top \;=\; \mb W^\star \mH^\star + (\mb W^\star \valpha + \widetilde\vb^\star)\mb 1^\top \;=\; \mW^\star\mH^\star.
\end{align*}
Therefore, we can see that $(\wt{\mW}^\star,\widetilde\mH^\star,\widetilde\vb^\star)$ achieves the same cross-entropy loss as $(\mW^\star,\mH^\star,\vb^\star)$. \zz{We can't say it is a global solution of $f$ it includes weight decay on the features, even we remove the weight decay for the bias term.}
\end{proof}
\end{comment}

%Here, the bias term in the last fully connected layer is included in the unconstrained feature model \eqref{eq:obj}, and our result indicates that a collapsing phenomenon also exists in the bias term $\vb^\star$ in the sense that all the elements of $\vb^\star$ are identical to each other. This suggests that removing the bias term $\vb$ causes no effect in the unconstrained feature model since the bias term with identical elements has no influence to the performance of the classifier. In the case that the features $\mH$ are nonnegative, such as a ReLu unit is applied at the end of the penultimate layer, the mean of the features $\overline \vh_i^\star$ will no longer be zero, but may contain positive elements. In this case, the bias term will play a role of compensating for the global mean of the features. %one may still prove similar neural collapse phenomenon for the global solution of the unconstrained feature model with nonnegative features. 


%Also, as explained in \eqref{eq:obj}, we assume the number of training samples in each class is balanced, for which the neural collapse is observed in \cite{papyan2020prevalence}. Next, we show that the Simplex ETF are the only global minimizers, and there is no other spurious bad local minimizer on the optimization landscape.  

%In \Cref{sec:experiment}, we will show empirical results suggesting that $(i)$ removing the bias term in the last fully connect layer causes little or no decline in classification performance for neural networks with arbitrary features, and $(ii)$ the bias term in the last fully connect layer compensates the global mean of the features for neural networks with nonnegative features. \zz{To remove the last sentence if no experiments are provided. Remove the first point since we will not have the experiments.} 

%the features of each class collapse to one point and any pair of features from different classes have an equal-sized angle

%========================

%

%=================================

%\Cref{thm:global-minima} shows that any global solution of the objective function in \eqref{eq:obj} exhibits neural collapse as the features of each class collapse to one point and any pair of features from different classes have an equal-sized angle,  %Throughout the paper, we consider the case where the feature dimension $d$ is larger than the number of classes $K$, which holds in the practice of deep learning. For example, the feature dimension is \zzedit{256 in ResNet18, a typical network for CIFAR10, and is 2048 in ResNet50, a typical network for ImageNet}. 
%\cy{The requirement that $d \ge K$ is necessary for the conclusion of \Cref{thm:global-minima} to hold, since $K$ vectors in $\bb R^d$ cannot form a $K$-Simplex ETF if $d < K$. In the practice of deep learning, $d$ is typically taken to be significantly larger than $K$. For example, the feature dimension $d$ of ResNet \cite{he2016deep} is 64 for CIFAR10, a dataset with $K = 10$ classes, and is 2048 for ImageNet, a dataset with $K = 1000$ classes. }
%The requirement that $d \ge K$ is necessary for the conclusion of \Cref{thm:global-minima} to hold, since $K$ vectors in $\bb R^d$ cannot form a $K$-Simplex ETF if $d < K$. 
%In the practice of deep learning, $d$ is typically taken to be significantly larger than $K$. For example, the feature dimension $d$ of ResNet \cite{he2016deep} is 64 for CIFAR10, a dataset with $K = 10$ classes, and is 2048 for ImageNet, a dataset with $K = 1000$ classes.
%Also, as explained in \eqref{eq:obj}, we assume the number of training samples in each class is balanced, for which the neural collapse is observed in \cite{papyan2020prevalence}. Next, we show that the Simplex ETF are the only global minimizers, and there is no other spurious bad local minimizer on the optimization landscape.  


%Similar results are also obtained in \cite{fang2021layer,lu2020neural,weinan2020emergence} which considered slightly different models, as described above. 

%assuming no weight decay on the bias term,

%In \Cref{sec:experiment}, we will show empirical results suggesting that removing the bias term in the last fully connect layer causes little or no decline in classification performance for common datasets such as MNIST and Cifar. 



%\js{I believe the equation for $\ol{\mb h}_{i}$ above implicitly assumes that $n_k=n ~\forall ~k$; i.e. that all classes have the same number of samples. I don't think this has been said.}\zz{Yes, we assume the balanced case in \eqref{eq:obj}. Also add a comment after \Cref{thm:global-minima}.}

\subsection{Characterizations of the Benign Global Landscape for \eqref{eq:obj}}\label{subsec:main-geometry}

The global optimality condition in \Cref{thm:global-minima} does not necessarily mean that we can achieve these global solutions efficiently, as the problem is still nonconvex. We now investigate the global optimization landscape of \eqref{eq:obj} by characterizing all of its critical points. Our next result implies that the training loss is a strict saddle function, and every critical point is either a global minimizer or a strict saddle point that can be escaped using negative curvatures. As a consequence, this implies that the global solutions of the training problem in \eqref{eq:obj} can be efficiently found from random initializations.


\begin{theorem}[No Spurious Local Minima and Strict Saddle Property]\label{thm:global-geometry}
		Assume that the feature dimension is larger than the number of classes, $d> K$, and the number of training samples in each class is balanced $n = n_1 = \cdots = n_K$. Then the function $f(\mb W,\mb H,\mb b)$ in \eqref{eq:obj} is a strict saddle function with no spurious local minimum, in the sense that
		
%	\vspace{-.1in}
	\begin{itemize}[leftmargin=*]
	%\setlength\itemsep{-0.05in}
	    \item Any local minimizer of \eqref{eq:obj} is a global minimizer of the form shown in \Cref{thm:global-minima}.
	    \item Any critical point $(\mb W,\mb H,\mb b)$ of \eqref{eq:obj} that is not a local minimizer is a strict saddle with negative curvature, i.e. the Hessian $\nabla^2 f(\mb W,\mb H,\mb b)$, at this critical point, is non-degenerate and has at least one negative eigenvalue, i.e. $\exists~ i : ~\lambda_i\paren{\nabla^2 f(\mb W,\mb H,\mb b)}<0$.
	\end{itemize}
\end{theorem}

%\qq{intuition behind creating the negative curvature direction, cite the paper: Loss Landscapes of Regularized Linear Autoencoders, make some connection to low-rank sensing, implicit bias for low-rank matrix factorization }


In a nutshell, our proof relies on connecting the original nonconvex optimization problem \eqref{eq:obj} to its corresponding low-rank convex counterpart, so that we can obtain the global optimality conditions for  \eqref{eq:obj} based on the latter. With this, we can then characterize the properties of all critical points based on the optimality conditions. We defer all details of this proof to Appendix \ref{app:thm-global}.

%\paragraph{Remark.} 
Existing results \cite{fang2021layer,lu2020neural,weinan2020emergence} have \emph{only} studied the global minimizers of the original problem, which has limited implication for optimization. In contrast, \Cref{thm:global-geometry} characterizes the properties for {\it all} critical points of the function in \eqref{eq:obj}. As a consequence of this result, many first-order and second-order optimization methods \cite{bottou2018optimization} optimizing $(\mb W,\mb H,\mb b)$ are guaranteed to converge to a global solution of \eqref{eq:obj}. In particular, the result in \cite{ge2015escaping,lee2016gradient} ensures that (stochastic) gradient descent with random initialization, the \emph{de facto} optimization algorithm used in deep learning, almost surely escapes strict saddles and converges to a second-order critical point -- which happens to be a global minimizer of form showed in \Cref{thm:global-minima} for our problem \eqref{eq:obj}.

\vspace{-.1in}
\begin{itemize}[leftmargin=*]
    \item \textbf{Constructing the Negative Curvature Direction for Strict Saddles. }%\js{not a big fan of "cooking", how about "finding"?} 
     One of the major difficulties in our proof is to construct the negative curvature direction for strict saddle points. Here, we exploit the fact that the feature dimension $d$ is larger than the number of classes $K$, and construct the negative curvature direction within the null space of $\mW \in \bb R^{K \times d}$. This is also the main reason for the requirement $d>K$ in \Cref{thm:global-geometry}, but we conjecture the results also hold for $d= K$ and could be proved with more sophisticated analysis, which is left as future work.
    \item \textbf{Relationship to Low-Rank Matrix Recovery.} As discussed in \revise{\Cref{sec:prior}}, it has been recently shown that the strict saddle property holds for a wide range of nonconvex problems in machine learning \cite{qu2014finding,zhao2015nonconvex,sun2016complete1,sun2015complete,li2016,qu2017convolutional,sun2018geometric,zhu2018global,li2019symmetry,zhu2018distributed,chi2019nonconvex,qu2020geometric,qu2020finding,qu2020exact}, including low-rank matrix recovery \cite{ge2016matrix,bhojanapalli2016global,ge2017no,li2019non,li2019symmetry,chi2019nonconvex}. 
   As we know that $\norm{\mb Z}{*} \;=\; \min_{ \mb Z = \mb W \mb H } \; \frac{1}{ 2  } (\norm{\mb W}{F}^2 +  \norm{\mb H}{F}^2)$ (see \cite{haeffele2015global} for a proof), our formulation in \eqref{eq:obj} is closely related to low-rank matrix problems \cite{ge2016matrix,bhojanapalli2016global,ge2017no,li2019non,li2019symmetry,chi2019nonconvex} with the Burer-Moneirto factorization approach \cite{burer2003nonlinear}, by viewing $\mW$ and $\mH$ as two factors of a matrix $\mb Z = \mb W \mb H $. The differences lie in the loss functions and statistical properties of the problem.\footnote{We consider the cross-entropy loss rather than the least-squares loss due to the differences in the task -- we focus on classification instead of recovery problems. On the other hand, the results on low-rank matrix recovery are often based on certain statistical properties, such as the randomness in the measurements \cite{ge2016matrix,bhojanapalli2016global}, or restricted well-conditionedness property of the objective function~\cite{zhu2018global,li2019non}. In contrast, these statistical properties do not exist in our problem, where the model and analysis are purely deterministic.} Thus, our result establishes a connection between the study of low-rank matrix factorization and neural networks under the unconstrained feature model.
    \item \textbf{Comparison to Existing Landscape Analysis on Neural Network.} \Cref{sec:intro} provided a comprehensive discussion on the relationship between our result and previous works on landscape analysis for deep neural networks. Although the unconstrained feature model can be viewed as a two-layer linear network with input being the columns of an identity matrix, as preluded in \Cref{sec:intro}, our result has much broader implications than the previous results \cite{baldi1989neural,kawaguchi2016deep,nouiehed2018learning,yun2018global,laurent2018deep,kunin2019loss,zhu2019global}. First, our problem formulation \eqref{eq:obj} is closer to practical settings for classification tasks, which considers the widely adopted cross-entropy loss while including weight decay and a bias term, while most existing results~\cite{baldi1989neural,kawaguchi2016deep,nouiehed2018learning,yun2018global,laurent2018deep,kunin2019loss,zhu2019global} either do not incorporate any regularization and bias, or focus on the squared loss for the regression problem. More importantly, our result characterizes the precise form of the global solutions (i.e., \NC) for the last layer features and classifiers, and shows that they can be efficiently achieved. Moreover, convincing numerical results in \cite{papyan2020prevalence} and the next section demonstrate that the global solutions do appear and can be achieved by practical networks on various standard image datasets. %\js{I'm a bit confused by the previous sentence: do you mean that that this has been extensively studied as in Papyan et al, or that this is what we will show in the next section?} 
    Our study of last-layer features could have profound implications for studying generalization and robustness of the deep networks.
\end{itemize}

 %Instead, we exploit the fact that the feature dimension is larger than the number of classes, and construct the negative curvature direction within the null space of $\mW$ for all the critical points that are not global solutions. We note that this is also the main reason for the requirement $d>K$ in \Cref{thm:global-geometry}, but we conjecture the results also hold for $d= k$ and can be proved with more sophisticated analysis, which is left as future work. %\zz{With this descrption, we may change the assumption in \Cref{thm:global-minima} to $d\ge K$?} 


%    because previous results are focused on recovery problems while we are solving classification tasks, the choice of loss functions is quite different -- they are based on the least-squares rather than the cross entropy loss we studied here. Additionally, they often studied the problem under certain statistical properties\footnote{} that 


%difference from shallow two-layer network, connections to nonconvex low-rank matrix recovery \zz{I think this can be discussed when we formally introduce the peel-layered model.} \qq{good point}

==> NeurIPS_2022/macro.tex <==



\usepackage{amsmath,amssymb,amsbsy,amsfonts,amscd,bm,url,color,latexsym}
\usepackage[hidelinks]{hyperref}
%amsthm, graphicx,amsmath,,amssymb,
%\usepackage{paralist}
\usepackage[dvipsnames]{xcolor}
\usepackage{color}
\usepackage{graphicx}
\graphicspath{{./figs/}}
\usepackage{algorithm}
\usepackage{algorithmic}
\usepackage{comment}
\usepackage{multirow}
\usepackage{enumitem}
\usepackage{fancyhdr}
%\usepackage{cite}
%\usepackage{citesort}
\usepackage{cleveref}
\usepackage{subcaption}
\usepackage{authblk}
% Theorems
%\def \remarks {\noindent {\bf Remarks.}\ \ }
\newtheorem{thm}{Theorem}%[section] %(If you want theorem numbered
%\newtheorem{lemma}{Lemma}%[section] %%    with section number.
\newtheorem{cor}{Corollary}%[section]
\newtheorem{prop}{Proposition}%[section]
%\newtheorem{definition}{Definition}%[section]
\newtheorem{defi}{Definition}%[section]
\newtheorem{assum}{Assumption}
%\newtheorem*{goal}{Plan}
%\newtheorem{theorem}{Theorem}
\newtheorem{lem}{Lemma}
%\theoremstyle{remark}
%\newtheorem{remark}{Remark}
%\theoremstyle{problem}
%\newtheorem{problem}{Problem}

% fields
\renewcommand{\O}{\mathbb{O}}
\newcommand{\R}{\mathbb{R}}
\def \real    { \mathbb{R} }
\def \reals   { \mathbb{R} }
\def \Real {\mathbb{R}}
\newcommand{\C}{\mathbb{C}}
\def \complex{\mathbb{C}}
\def \Complex {\mathbb{C}}
\newcommand{\Z}{\mathbb{Z}}
\newcommand{\N}{\mathbb{N}}

\newcommand{\la}{\left\langle}
\newcommand{\ra}{\right\rangle}
\newcommand{\e}{\begin{equation}}
\newcommand{\ee}{\end{equation}}
\newcommand{\en}{\begin{equation*}}
\newcommand{\een}{\end{equation*}}
\newcommand{\eqn}{\begin{eqnarray}}
\newcommand{\eeqn}{\end{eqnarray}}
\newcommand{\bmat}{\begin{bmatrix}}
\newcommand{\emat}{\end{bmatrix}}
% complex numbers
\renewcommand{\Re}[1]{\operatorname{Re}\left\{#1\right\}}
\renewcommand{\Im}[1]{\operatorname{Im}\left\{#1\right\}}
\newcommand{\conj}[1]{\mkern 1.5mu\overline{\mkern-1.5mu#1\mkern-1.5mu}\mkern 1.5mu}

\DeclareMathAlphabet\mathbfcal{OMS}{cmsy}{b}{n}
% probability and stat
\renewcommand{\P}[1]{\operatorname{\mathbb{P}}\left(#1\right)}
\newcommand{\E}{\operatorname{\mathbb{E}}}
\newcommand{\dif}{\operatorname{d}}
\newcommand{\var}{\operatorname{var}}

% calculus
\renewcommand{\d}[1]{\,\mathrm{d}#1}

% constants (written in roman, if wanted)
%\newcommand{\e}{\mathrm{e}}
\renewcommand{\j}{\mathrm{j}}




\newcommand{\mb}{\mathbf}
\newcommand{\mc}{\mathcal}
\newcommand{\mf}{\mathfrak}
\newcommand{\bb}{\mathbb}
\newcommand{\mrm}{\mathrm}
\newcommand{\mtt}{\mathtt}
\def \vecword  {\operatorname*{vec}}
% linear algebra
% 	vector notation
\newcommand{\vct}[1]{\boldsymbol{#1}}
%   matrices
\newcommand{\mtx}[1]{\boldsymbol{#1}}
%   block vector
\newcommand{\bvct}[1]{\mathbf{#1}}
%   block matrix
\newcommand{\bmtx}[1]{\mathbf{#1}}
%	inner products
\newcommand{\inner}[1]{\left<#1\right>}
\newcommand{\<}{\langle}
\renewcommand{\>}{\rangle}
% 	transpose, Hermitian, pseudo-inverse
\renewcommand{\H}{\mathrm{H}}
\newcommand{\T}{\mathrm{T}}
\newcommand{\pinv}{\dagger}
%	fundamental subspaces
\newcommand{\Null}{\operatorname{Null}}
\newcommand{\Range}{\operatorname{Range}}
\newcommand{\Span}{\operatorname{Span}}
%	operators
\newcommand{\trace}{\operatorname{trace}}
\newcommand{\conv}{\operatorname{conv}}
\newcommand{\rank}{\operatorname{rank}}
\newcommand{\diag}{\operatorname{diag}}
\newcommand{\toep}{\operatorname{Toep}}
\newcommand{\SDP}{\operatorname{SDP}}
\newcommand{\PSD}{\operatorname{PSD}}
\newcommand{\far}{\operatorname{far}}
\newcommand{\near}{\operatorname{near}}
\newcommand{\sign}{\operatorname{sign}}
\newcommand{\sgn}{\operatorname{sgn}}
\newcommand{\Sign}{\operatorname{Sgn}}
\newcommand{\dist}{\operatorname{dist}}
\def \lg        {\langle}
\def \rg        {\rangle}
\def \vec       {\operatorname*{vec}}
%
\newcommand{\dimension}{\operatorname{dim}}

% sets and topology
\newcommand{\set}[1]{\mathbb{#1}}
\newcommand{\closure}{\operatorname{cl}}	% closure
\newcommand{\interior}{\operatorname{int}}
\newcommand{\boundary}{\operatorname{bd}}
\newcommand{\diameter}{\operatorname{diam}}

% functional analysis
\newcommand{\domain}{\operatorname{dom}}
\newcommand{\epigraph}{\operatorname{epi}}
\newcommand{\hypograph}{\operatorname{hypo}}
\newcommand{\linop}[1]{\mathscr{#1}}	% general linear operator

% optimization
\DeclareMathOperator*{\minimize}{\text{minimize}}
\DeclareMathOperator*{\maximize}{\text{maximize}}
\DeclareMathOperator*{\argmin}{\text{arg~min}}
\DeclareMathOperator*{\argmax}{\text{arg~max}}
\def \st {\operatorname*{s.t.\ }}
% other
%\newcommand{\sgn}{\text{sgn}}
\newcommand{\sinc}{\text{sinc}}
\newcommand{\floor}[1]{\left\lfloor #1 \right\rfloor}
\newcommand{\ceil}[1]{\left\lceil #1 \right\rceil}
\newcommand{\eps}{\epsilon}


\newcommand{\wh}{\widehat}
\newcommand{\wc}{\widecheck}
\newcommand{\wt}{\widetilde}
\newcommand{\ol}{\overline}
\newcommand{\NC}{$\mc {NC}$}

\newcommand{\norm}[2]{\left\| #1 \right\|_{#2}}
\newcommand{\nrm}[1]{\left\Vert#1\right\Vert}
\newcommand{\abs}[1]{\left| #1 \right|}
\newcommand{\bracket}[1]{\left( #1 \right)}
\newcommand{\parans}[1]{\left(#1\right)}
\newcommand{\innerprod}[2]{\left\langle #1,  #2 \right\rangle}
\newcommand{\prob}[1]{\bb P\left[ #1 \right]}
\newcommand{\expect}[1]{\bb E\left[ #1 \right]}
\newcommand{\function}[2]{#1 \left(#2\right)}
\newcommand{\integral}[4]{\int_{#1}^{#2}\; #3\; #4}
\newcommand{\iter}[1]{^{(#1)}}
\newcommand*\samethanks[1][\value{footnote}]{\footnotemark[#1]}

\newcommand{\js}[1]{{\color{blue} [\noindent JS: #1]}}

%--------------------------------------------------------------------------
\newcommand{\calA}{\mathcal{A}}
\newcommand{\calB}{\mathcal{B}}
\newcommand{\calC}{\mathcal{C}}
\newcommand{\calD}{\mathcal{D}}
\newcommand{\calE}{\mathcal{E}}
\newcommand{\calF}{\mathcal{F}}
\newcommand{\calG}{\mathcal{G}}
\newcommand{\calH}{\mathcal{H}}
\newcommand{\calI}{\mathcal{I}}
\newcommand{\calJ}{\mathcal{J}}
\newcommand{\calK}{\mathcal{K}}
\newcommand{\calL}{\mathcal{L}}
\newcommand{\calM}{\mathcal{M}}
\newcommand{\calN}{\mathcal{N}}
\newcommand{\calO}{\mathcal{O}}
\newcommand{\calP}{\mathcal{P}}
\newcommand{\calQ}{\mathcal{Q}}
\newcommand{\calR}{\mathcal{R}}
\newcommand{\calS}{\mathcal{S}}
\newcommand{\calT}{\mathcal{T}}
\newcommand{\calU}{\mathcal{U}}
\newcommand{\calV}{\mathcal{V}}
\newcommand{\calW}{\mathcal{W}}
\newcommand{\calX}{\mathcal{X}}
\newcommand{\calY}{\mathcal{Y}}
\newcommand{\calZ}{\mathcal{Z}}





\newcommand{\va}{\vct{a}}
\newcommand{\vb}{\vct{b}}
\newcommand{\vc}{\vct{c}}
\newcommand{\vd}{\vct{d}}
\newcommand{\ve}{\vct{e}}
\newcommand{\vf}{\vct{f}}
\newcommand{\vg}{\vct{g}}
\newcommand{\vh}{\vct{h}}
\newcommand{\vi}{\vct{i}}
\newcommand{\vj}{\vct{j}}
\newcommand{\vk}{\vct{k}}
\newcommand{\vl}{\vct{l}}
\newcommand{\vm}{\vct{m}}
\newcommand{\vn}{\vct{n}}
\newcommand{\vo}{\vct{o}}
\newcommand{\vp}{\vct{p}}
\newcommand{\vq}{\vct{q}}
\newcommand{\vr}{\vct{r}}
\newcommand{\vs}{\vct{s}}
\newcommand{\vt}{\vct{t}}
\newcommand{\vu}{\vct{u}}
\newcommand{\vv}{\vct{v}}
\newcommand{\vw}{\vct{w}}
\newcommand{\vx}{\vct{x}}
\newcommand{\vy}{\vct{y}}
\newcommand{\vz}{\vct{z}}
%
\newcommand{\valpha}{\vct{\alpha}}
\newcommand{\vbeta}{\vct{\beta}}
\newcommand{\vtheta}{\vct{\theta}}
\newcommand{\vepsilon}{\vct{\epsilon}}
\newcommand{\veps}{\vct{\epsilon}}
\newcommand{\vvarepsilon}{\vct{\varepsilon}}
\newcommand{\vgamma}{\vct{\gamma}}
\newcommand{\vlambda}{\vct{\lambda}}
\newcommand{\vnu}{\vct{\nu}}
\newcommand{\vphi}{\vct{\phi}}
\newcommand{\vpsi}{\vct{\psi}}
\newcommand{\vdelta}{\vct{\delta}}
\newcommand{\veta}{\vct{\eta}}
\newcommand{\vxi}{\vct{\xi}}
\newcommand{\vmu}{\vct{\mu}}
\newcommand{\vrho}{\vct{\rho}}
%
\newcommand{\vzero}{\vct{0}}
\newcommand{\vone}{\vct{1}}


\newcommand{\mA}{\mtx{A}}
\newcommand{\mB}{\mtx{B}}
\newcommand{\mC}{\mtx{C}}
\newcommand{\mD}{\mtx{D}}
\newcommand{\mE}{\mtx{E}}
\newcommand{\mF}{\mtx{F}}
\newcommand{\mG}{\mtx{G}}
\newcommand{\mH}{\mtx{H}}
\newcommand{\mJ}{\mtx{J}}
\newcommand{\mK}{\mtx{K}}
\newcommand{\mL}{\mtx{L}}
\newcommand{\mM}{\mtx{M}}
\newcommand{\mN}{\mtx{N}}
\newcommand{\mO}{\mtx{O}}
\newcommand{\mP}{\mtx{P}}
\newcommand{\mQ}{\mtx{Q}}
\newcommand{\mR}{\mtx{R}}
\newcommand{\mS}{\mtx{S}}
\newcommand{\mT}{\mtx{T}}
\newcommand{\mU}{\mtx{U}}
\newcommand{\mV}{\mtx{V}}
\newcommand{\mW}{\mtx{W}}
\newcommand{\mX}{\mtx{X}}
\newcommand{\mY}{\mtx{Y}}
\newcommand{\mZ}{\mtx{Z}}
%
\newcommand{\mGamma}{\mtx{\Gamma}}
\newcommand{\mDelta}{\mtx{\Delta}}
\newcommand{\mLambda}{\mtx{\Lambda}}
\newcommand{\mOmega}{\mtx{\Omega}}
\newcommand{\mPhi}{\mtx{\Phi}}
\newcommand{\mPsi}{\mtx{\Psi}}
\newcommand{\mSigma}{\mtx{\Sigma}}
\newcommand{\mTheta}{\mtx{\Theta}}
\newcommand{\mUpsilon}{\mtx{\Upsilon}}
%
\newcommand{\mId}{\bmtx{I}}
\newcommand{\mEx}{{\bf J}}
\newcommand{\mzero}{{\bf 0}}
\newcommand{\mone}{{\bf 1}}
%
\newcommand{\bva}{\bvct{a}}
\newcommand{\bvh}{\bvct{h}}
\newcommand{\bvw}{\bvct{w}}
\newcommand{\bvx}{\bvct{x}}
\newcommand{\bvy}{\bvct{y}}


\newcommand{\bmM}{\bmtx{M}}
\newcommand{\bmH}{\bmtx{H}}
\newcommand{\bmX}{\bmtx{X}}


\newcommand{\setA}{\set{A}}
\newcommand{\setB}{\set{B}}
\newcommand{\setC}{\set{C}}
\newcommand{\setD}{\set{D}}
\newcommand{\setE}{\set{E}}
\newcommand{\setF}{\set{F}}
\newcommand{\setG}{\set{G}}
\newcommand{\setH}{\set{H}}
\newcommand{\setI}{\set{I}}
\newcommand{\setJ}{\set{J}}
\newcommand{\setK}{\set{K}}
\newcommand{\setL}{\set{L}}
\newcommand{\setM}{\set{M}}
\newcommand{\setN}{\set{N}}
\newcommand{\setO}{\set{O}}
\newcommand{\setP}{\set{P}}
\newcommand{\setQ}{\set{Q}}
\newcommand{\setR}{\set{R}}
\newcommand{\setS}{\set{S}}
\newcommand{\setT}{\set{T}}
\newcommand{\setU}{\set{U}}
\newcommand{\setV}{\set{V}}
\newcommand{\setW}{\set{W}}
\newcommand{\setX}{\set{X}}
\newcommand{\setY}{\set{Y}}
\newcommand{\setZ}{\set{Z}}

\renewcommand{\ss}{{\vspace*{-1mm}}}

\setcounter{MaxMatrixCols}{20}

%\pagestyle{plain}

\graphicspath{{./figs/}}

\newlength{\imgwidth}
\setlength{\imgwidth}{3.125in}

\newcommand{\QW}[1]{\textcolor{red}{\bf [{\em QW:} #1]}}
\newcommand{\note}[1]{\textcolor{blue}{\bf [{\em Note:} #1]}}
\newcommand{\revise}[1]{\textcolor{blue}{#1}}
\newcommand{\edit}[1]{\textcolor{red}{#1}}

\newboolean{twoColVersion}
\setboolean{twoColVersion}{false}
\newcommand{\twoCol}[2]{\ifthenelse{\boolean{twoColVersion}} {#1} {#2} }


\usepackage{tikz}
\usepackage{tikz-3dplot}
\usepackage{pgfplots}
\usepgfplotslibrary{patchplots}
\usetikzlibrary{patterns, positioning, arrows}
\pgfplotsset{compat=1.15}



==> NeurIPS_2022/macro_nips.tex <==



\usepackage{amsmath,amssymb,amsbsy,amsfonts,amscd,bm,url,color,latexsym}
\usepackage[hidelinks]{hyperref}
%amsthm, graphicx,amsmath,,amssymb,
%\usepackage{paralist}
\usepackage[dvipsnames]{xcolor}
\usepackage{color}
\usepackage{graphicx}
\graphicspath{{./figs/}}
\usepackage{algorithm}
\usepackage{algorithmic}
\usepackage{comment}
\usepackage{multirow}
\usepackage{enumitem}
\usepackage{fancyhdr}
\usepackage{cite}
%\usepackage{citesort}
\usepackage{cleveref}
\usepackage{subcaption}
%\usepackage{authblk}
% Theorems
%\def \remarks {\noindent {\bf Remarks.}\ \ }
\newtheorem{thm}{Theorem}%[section] %(If you want theorem numbered
%\newtheorem{lemma}{Lemma}%[section] %%    with section number.
\newtheorem{cor}{Corollary}%[section]
\newtheorem{prop}{Proposition}%[section]
%\newtheorem{definition}{Definition}%[section]
\newtheorem{defi}{Definition}%[section]
\newtheorem{assum}{Assumption}
%\newtheorem*{goal}{Plan}
%\newtheorem{theorem}{Theorem}
\newtheorem{lem}{Lemma}
%\theoremstyle{remark}
%\newtheorem{remark}{Remark}
%\theoremstyle{problem}
%\newtheorem{problem}{Problem}

% fields
\renewcommand{\O}{\mathbb{O}}
\newcommand{\R}{\mathbb{R}}
\def \real    { \mathbb{R} }
\def \reals   { \mathbb{R} }
\def \Real {\mathbb{R}}
\newcommand{\C}{\mathbb{C}}
\def \complex{\mathbb{C}}
\def \Complex {\mathbb{C}}
\newcommand{\Z}{\mathbb{Z}}
\newcommand{\N}{\mathbb{N}}

\newcommand{\la}{\left\langle}
\newcommand{\ra}{\right\rangle}
\newcommand{\e}{\begin{equation}}
\newcommand{\ee}{\end{equation}}
\newcommand{\en}{\begin{equation*}}
\newcommand{\een}{\end{equation*}}
\newcommand{\eqn}{\begin{eqnarray}}
\newcommand{\eeqn}{\end{eqnarray}}
\newcommand{\bmat}{\begin{bmatrix}}
\newcommand{\emat}{\end{bmatrix}}
% complex numbers
\renewcommand{\Re}[1]{\operatorname{Re}\left\{#1\right\}}
\renewcommand{\Im}[1]{\operatorname{Im}\left\{#1\right\}}
\newcommand{\conj}[1]{\mkern 1.5mu\overline{\mkern-1.5mu#1\mkern-1.5mu}\mkern 1.5mu}

\DeclareMathAlphabet\mathbfcal{OMS}{cmsy}{b}{n}
% probability and stat
\renewcommand{\P}[1]{\operatorname{\mathbb{P}}\left(#1\right)}
\newcommand{\E}{\operatorname{\mathbb{E}}}
\newcommand{\dif}{\operatorname{d}}
\newcommand{\var}{\operatorname{var}}

% calculus
\renewcommand{\d}[1]{\,\mathrm{d}#1}

% constants (written in roman, if wanted)
%\newcommand{\e}{\mathrm{e}}
\renewcommand{\j}{\mathrm{j}}




\newcommand{\mb}{\mathbf}
\newcommand{\mc}{\mathcal}
\newcommand{\mf}{\mathfrak}
\newcommand{\bb}{\mathbb}
\newcommand{\mrm}{\mathrm}
\newcommand{\mtt}{\mathtt}
\def \vecword  {\operatorname*{vec}}
% linear algebra
% 	vector notation
\newcommand{\vct}[1]{\boldsymbol{#1}}
%   matrices
\newcommand{\mtx}[1]{\boldsymbol{#1}}
%   block vector
\newcommand{\bvct}[1]{\mathbf{#1}}
%   block matrix
\newcommand{\bmtx}[1]{\mathbf{#1}}
%	inner products
\newcommand{\inner}[1]{\left<#1\right>}
\newcommand{\<}{\langle}
\renewcommand{\>}{\rangle}
% 	transpose, Hermitian, pseudo-inverse
\renewcommand{\H}{\mathrm{H}}
\newcommand{\T}{\mathrm{T}}
\newcommand{\pinv}{\dagger}
%	fundamental subspaces
\newcommand{\Null}{\operatorname{Null}}
\newcommand{\Range}{\operatorname{Range}}
\newcommand{\Span}{\operatorname{Span}}
%	operators
\newcommand{\trace}{\operatorname{trace}}
\newcommand{\conv}{\operatorname{conv}}
\newcommand{\rank}{\operatorname{rank}}
\newcommand{\diag}{\operatorname{diag}}
\newcommand{\toep}{\operatorname{Toep}}
\newcommand{\SDP}{\operatorname{SDP}}
\newcommand{\PSD}{\operatorname{PSD}}
\newcommand{\far}{\operatorname{far}}
\newcommand{\near}{\operatorname{near}}
\newcommand{\sign}{\operatorname{sign}}
\newcommand{\sgn}{\operatorname{sgn}}
\newcommand{\Sign}{\operatorname{Sgn}}
\newcommand{\dist}{\operatorname{dist}}
\def \lg        {\langle}
\def \rg        {\rangle}
\def \vec       {\operatorname*{vec}}
%
\newcommand{\dimension}{\operatorname{dim}}

% sets and topology
\newcommand{\set}[1]{\mathbb{#1}}
\newcommand{\closure}{\operatorname{cl}}	% closure
\newcommand{\interior}{\operatorname{int}}
\newcommand{\boundary}{\operatorname{bd}}
\newcommand{\diameter}{\operatorname{diam}}

% functional analysis
\newcommand{\domain}{\operatorname{dom}}
\newcommand{\epigraph}{\operatorname{epi}}
\newcommand{\hypograph}{\operatorname{hypo}}
\newcommand{\linop}[1]{\mathscr{#1}}	% general linear operator

% optimization
\DeclareMathOperator*{\minimize}{\text{minimize}}
\DeclareMathOperator*{\maximize}{\text{maximize}}
\DeclareMathOperator*{\argmin}{\text{arg~min}}
\DeclareMathOperator*{\argmax}{\text{arg~max}}
\def \st {\operatorname*{s.t.\ }}
% other
%\newcommand{\sgn}{\text{sgn}}
\newcommand{\sinc}{\text{sinc}}
\newcommand{\floor}[1]{\left\lfloor #1 \right\rfloor}
\newcommand{\ceil}[1]{\left\lceil #1 \right\rceil}
\newcommand{\eps}{\epsilon}


\newcommand{\wh}{\widehat}
\newcommand{\wc}{\widecheck}
\newcommand{\wt}{\widetilde}
\newcommand{\ol}{\overline}
\newcommand{\NC}{$\mc {NC}$}

\newcommand{\norm}[2]{\left\| #1 \right\|_{#2}}
\newcommand{\nrm}[1]{\left\Vert#1\right\Vert}
\newcommand{\abs}[1]{\left| #1 \right|}
\newcommand{\bracket}[1]{\left( #1 \right)}
\newcommand{\parans}[1]{\left(#1\right)}
\newcommand{\innerprod}[2]{\left\langle #1,  #2 \right\rangle}
\newcommand{\prob}[1]{\bb P\left[ #1 \right]}
\newcommand{\expect}[1]{\bb E\left[ #1 \right]}
\newcommand{\function}[2]{#1 \left(#2\right)}
\newcommand{\integral}[4]{\int_{#1}^{#2}\; #3\; #4}
\newcommand{\iter}[1]{^{(#1)}}
\newcommand*\samethanks[1][\value{footnote}]{\footnotemark[#1]}

\newcommand{\js}[1]{{\color{blue} [\noindent JS: #1]}}

%--------------------------------------------------------------------------
\newcommand{\calA}{\mathcal{A}}
\newcommand{\calB}{\mathcal{B}}
\newcommand{\calC}{\mathcal{C}}
\newcommand{\calD}{\mathcal{D}}
\newcommand{\calE}{\mathcal{E}}
\newcommand{\calF}{\mathcal{F}}
\newcommand{\calG}{\mathcal{G}}
\newcommand{\calH}{\mathcal{H}}
\newcommand{\calI}{\mathcal{I}}
\newcommand{\calJ}{\mathcal{J}}
\newcommand{\calK}{\mathcal{K}}
\newcommand{\calL}{\mathcal{L}}
\newcommand{\calM}{\mathcal{M}}
\newcommand{\calN}{\mathcal{N}}
\newcommand{\calO}{\mathcal{O}}
\newcommand{\calP}{\mathcal{P}}
\newcommand{\calQ}{\mathcal{Q}}
\newcommand{\calR}{\mathcal{R}}
\newcommand{\calS}{\mathcal{S}}
\newcommand{\calT}{\mathcal{T}}
\newcommand{\calU}{\mathcal{U}}
\newcommand{\calV}{\mathcal{V}}
\newcommand{\calW}{\mathcal{W}}
\newcommand{\calX}{\mathcal{X}}
\newcommand{\calY}{\mathcal{Y}}
\newcommand{\calZ}{\mathcal{Z}}





\newcommand{\va}{\vct{a}}
\newcommand{\vb}{\vct{b}}
\newcommand{\vc}{\vct{c}}
\newcommand{\vd}{\vct{d}}
\newcommand{\ve}{\vct{e}}
\newcommand{\vf}{\vct{f}}
\newcommand{\vg}{\vct{g}}
\newcommand{\vh}{\vct{h}}
\newcommand{\vi}{\vct{i}}
\newcommand{\vj}{\vct{j}}
\newcommand{\vk}{\vct{k}}
\newcommand{\vl}{\vct{l}}
\newcommand{\vm}{\vct{m}}
\newcommand{\vn}{\vct{n}}
\newcommand{\vo}{\vct{o}}
\newcommand{\vp}{\vct{p}}
\newcommand{\vq}{\vct{q}}
\newcommand{\vr}{\vct{r}}
\newcommand{\vs}{\vct{s}}
\newcommand{\vt}{\vct{t}}
\newcommand{\vu}{\vct{u}}
\newcommand{\vv}{\vct{v}}
\newcommand{\vw}{\vct{w}}
\newcommand{\vx}{\vct{x}}
\newcommand{\vy}{\vct{y}}
\newcommand{\vz}{\vct{z}}
%
\newcommand{\valpha}{\vct{\alpha}}
\newcommand{\vbeta}{\vct{\beta}}
\newcommand{\vtheta}{\vct{\theta}}
\newcommand{\vepsilon}{\vct{\epsilon}}
\newcommand{\veps}{\vct{\epsilon}}
\newcommand{\vvarepsilon}{\vct{\varepsilon}}
\newcommand{\vgamma}{\vct{\gamma}}
\newcommand{\vlambda}{\vct{\lambda}}
\newcommand{\vnu}{\vct{\nu}}
\newcommand{\vphi}{\vct{\phi}}
\newcommand{\vpsi}{\vct{\psi}}
\newcommand{\vdelta}{\vct{\delta}}
\newcommand{\veta}{\vct{\eta}}
\newcommand{\vxi}{\vct{\xi}}
\newcommand{\vmu}{\vct{\mu}}
\newcommand{\vrho}{\vct{\rho}}
%
\newcommand{\vzero}{\vct{0}}
\newcommand{\vone}{\vct{1}}


\newcommand{\mA}{\mtx{A}}
\newcommand{\mB}{\mtx{B}}
\newcommand{\mC}{\mtx{C}}
\newcommand{\mD}{\mtx{D}}
\newcommand{\mE}{\mtx{E}}
\newcommand{\mF}{\mtx{F}}
\newcommand{\mG}{\mtx{G}}
\newcommand{\mH}{\mtx{H}}
\newcommand{\mJ}{\mtx{J}}
\newcommand{\mK}{\mtx{K}}
\newcommand{\mL}{\mtx{L}}
\newcommand{\mM}{\mtx{M}}
\newcommand{\mN}{\mtx{N}}
\newcommand{\mO}{\mtx{O}}
\newcommand{\mP}{\mtx{P}}
\newcommand{\mQ}{\mtx{Q}}
\newcommand{\mR}{\mtx{R}}
\newcommand{\mS}{\mtx{S}}
\newcommand{\mT}{\mtx{T}}
\newcommand{\mU}{\mtx{U}}
\newcommand{\mV}{\mtx{V}}
\newcommand{\mW}{\mtx{W}}
\newcommand{\mX}{\mtx{X}}
\newcommand{\mY}{\mtx{Y}}
\newcommand{\mZ}{\mtx{Z}}
%
\newcommand{\mGamma}{\mtx{\Gamma}}
\newcommand{\mDelta}{\mtx{\Delta}}
\newcommand{\mLambda}{\mtx{\Lambda}}
\newcommand{\mOmega}{\mtx{\Omega}}
\newcommand{\mPhi}{\mtx{\Phi}}
\newcommand{\mPsi}{\mtx{\Psi}}
\newcommand{\mSigma}{\mtx{\Sigma}}
\newcommand{\mTheta}{\mtx{\Theta}}
\newcommand{\mUpsilon}{\mtx{\Upsilon}}
%
\newcommand{\mId}{\bmtx{I}}
\newcommand{\mEx}{{\bf J}}
\newcommand{\mzero}{{\bf 0}}
\newcommand{\mone}{{\bf 1}}
%
\newcommand{\bva}{\bvct{a}}
\newcommand{\bvh}{\bvct{h}}
\newcommand{\bvw}{\bvct{w}}
\newcommand{\bvx}{\bvct{x}}
\newcommand{\bvy}{\bvct{y}}


\newcommand{\bmM}{\bmtx{M}}
\newcommand{\bmH}{\bmtx{H}}
\newcommand{\bmX}{\bmtx{X}}


\newcommand{\setA}{\set{A}}
\newcommand{\setB}{\set{B}}
\newcommand{\setC}{\set{C}}
\newcommand{\setD}{\set{D}}
\newcommand{\setE}{\set{E}}
\newcommand{\setF}{\set{F}}
\newcommand{\setG}{\set{G}}
\newcommand{\setH}{\set{H}}
\newcommand{\setI}{\set{I}}
\newcommand{\setJ}{\set{J}}
\newcommand{\setK}{\set{K}}
\newcommand{\setL}{\set{L}}
\newcommand{\setM}{\set{M}}
\newcommand{\setN}{\set{N}}
\newcommand{\setO}{\set{O}}
\newcommand{\setP}{\set{P}}
\newcommand{\setQ}{\set{Q}}
\newcommand{\setR}{\set{R}}
\newcommand{\setS}{\set{S}}
\newcommand{\setT}{\set{T}}
\newcommand{\setU}{\set{U}}
\newcommand{\setV}{\set{V}}
\newcommand{\setW}{\set{W}}
\newcommand{\setX}{\set{X}}
\newcommand{\setY}{\set{Y}}
\newcommand{\setZ}{\set{Z}}

\renewcommand{\ss}{{\vspace*{-1mm}}}

\setcounter{MaxMatrixCols}{20}

%\pagestyle{plain}

\graphicspath{{./figs/}}

\newlength{\imgwidth}
\setlength{\imgwidth}{3.125in}

\newcommand{\QW}[1]{\textcolor{red}{\bf [{\em QW:} #1]}}
\newcommand{\note}[1]{\textcolor{blue}{\bf [{\em Note:} #1]}}
\newcommand{\edit}[1]{\textcolor{red}{#1}}

\newboolean{twoColVersion}
\setboolean{twoColVersion}{false}
\newcommand{\twoCol}[2]{\ifthenelse{\boolean{twoColVersion}} {#1} {#2} }


\newcommand{\Poff}{\mathcal{P}_{\textup{off}}}
\newcommand{\Pon}{\mathcal{P}_{\textup{diag}}}

\usepackage{tikz}
\usepackage{tikz-3dplot}
\usepackage{pgfplots}
\usepgfplotslibrary{patchplots}
\usetikzlibrary{patterns, positioning, arrows}
\pgfplotsset{compat=1.15}



%\usepackage{tgpagella}
%\usepackage[utf8]{inputenc} % allow utf-8 input
%\usepackage[T1]{fontenc}    % use 8-bit T1 fonts

\usepackage{url}
%\usepackage{hyperref}       % hyperlinks
%\usepackage{url}            % simple URL typesetting
%\usepackage{booktabs}       % professional-quality tables
%\usepackage{nicefrac}       % compact symbols for 1/2, etc.
%\usepackage{microtype}      % microtypography
%\usepackage{authblk}
%\usepackage{multirow}
%\usepackage{mathabx}

%\usepackage{graphicx,amsmath,amsfonts,amscd,amssymb,bm,url,color,latexsym}
%\usepackage[margin=0.95in]{geometry}

%\usepackage[inline]{enumitem}
%\usepackage{mwe}
%\usepackage{subfigure}
%\usepackage{subfig}
%\usepackage{subcaption}
%\usepackage{bbm}
%\usepackage{bm}
%\usepackage{microtype}
%\setlength{\captionmargin}{30pt}
%\usepackage{algorithm,algorithmicx}
%\usepackage{algpseudocode}
%\usepackage{hyperref}
%\usepackage[nameinlink]{cleveref}
%\usepackage{verbatim}
%\usepackage{framed}
%\usepackage{comment}
%\usepackage{wrapfig}
%\usepackage{tikz}
%\usepackage{pgfplots}

%\usepackage{cite}
%\usepackage{tikz}
%\usepackage{multirow}
%\usepackage{cleveref}

%\usepackage{tablefootnote}
%\usepackage{tcolorbox}
%\usepackage{pifont}
%\usepackage{authblk}
%\usepackage[margin=0.95in]{geometry}

\providecommand{\keywords}[1]{\textbf{\textit{Index terms---}} #1}


% pagebreak for long equations
%\allowdisplaybreaks

\hypersetup{
    colorlinks=true,%
    citecolor=blue,%
    filecolor=blue,%
    linkcolor=blue,%
    urlcolor=blue
}
\usepackage[toc, page]{appendix}
%%%%%%%%%%%%%%
\renewcommand\floatpagefraction{.95}
\renewcommand\topfraction{.95}
\renewcommand\bottomfraction{.95}
\renewcommand\textfraction{.05}
\setcounter{totalnumber}{50}
\setcounter{topnumber}{50}
\setcounter{bottomnumber}{50}
%%%%%%%%%%%%%%
%--------------
\newtheorem{theorem}{Theorem}[section]
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{conjecture}[theorem]{Conjecture}
%\newtheorem{problem}[theorem]{Problem}
%\newtheorem{claim}[theorem]{Claim}
\newtheorem{remark}[theorem]{Remark}
%\newtheorem{example}[theorem]{Example}
%\newtheorem{assumption}[theorem]{Assumption}


\newcommand{\indep}{\rotatebox[origin=c]{90}{$\models$}}

\renewcommand{\mathbf}{\boldsymbol}

%\newcommand{\conv}{\circledast}
\newcommand{\cconv}{  \boxasterisk }
%\newcommand{\mb}{\mathbf}
%\newcommand{\mc}{\mathcal}
%\newcommand{\mf}{\mathfrak}
\newcommand{\md}{\mathds}
%\newcommand{\bb}{\mathbb}
\newcommand{\magnitude}[1]{ \left| #1 \right| }
%\newcommand{\set}[1]{\left\{ #1 \right\}}
\newcommand{\condset}[2]{ \left\{ #1 \;\middle|\; #2 \right\} }



%\newcommand{\reals}{\bb R}
\newcommand{\proj}{\mathrm{proj}}
%\newcommand{\E}{\mathbb{E}}

%\newcommand{\eps}{\varepsilon}
%\newcommand{\R}{\reals}
\newcommand{\Cp}{\bb C}
%\newcommand{\Z}{\bb Z}
%\newcommand{\N}{\bb N}
\newcommand{\Sp}{\bb S}
\newcommand{\Ba}{\bb B}
\newcommand{\indicator}[1]{\mathbbm 1_{#1}}
\renewcommand{\P}{\mathbb{P}}

\newcommand{ \Brac }[1]{\left\lbrace #1 \right\rbrace}
\newcommand{ \brac }[1]{\left[ #1 \right]}
\newcommand{ \paren }[1]{ \left( #1 \right) }
\newcommand{\col}{\mathrm{col}}

\newcommand{\Lce}{\mc L_{\mathrm{CE}}}

% to declare new operator
% \DeclareMathOperator{\xxx}{xxx}
%\DeclareMathOperator{\dist}{dist}
\DeclareMathOperator{\poly}{poly}
%\DeclareMathOperator{\rank}{rank}
%\DeclareMathOperator{\trace}{tr}
\DeclareMathOperator{\supp}{supp}
\DeclareMathOperator{\vect}{vec}
%\DeclareMathOperator{\diag}{diag}
%\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\grad}{grad}
\DeclareMathOperator{\Hess}{Hess}
\DeclareMathOperator{\mini}{minimize}
\DeclareMathOperator{\maxi}{maximize}
%\DeclareMathOperator{\st}{subject\; to}

%% Other definitions


%\newcommand{\wh}{\widehat}
%\newcommand{\wt}{\widetilde}
%\newcommand{\ol}{\overline}
%\newcommand{\wc}{\widecheck}



%\newcommand{\norm}[2]{\left\| #1 \right\|_{#2}}
%\newcommand{\abs}[1]{\left| #1 \right|}
%\newcommand{\innerprod}[2]{\left\langle #1,  #2 \right\rangle}
%\newcommand{\prob}[1]{\bb P\left[ #1 \right]}
%\newcommand{\expect}[1]{\bb E\left[ #1 \right]}
%\newcommand{\function}[2]{#1 \left(#2\right)}
%\newcommand{\integral}[4]{\int_{#1}^{#2}\; #3\; #4}


%\newcommand{ \vphi }[1]{ \varphi( #1 ) }
%\newcommand{ \vphiT }[1]{ \varphi_{\mathrm{T}}( #1 ) }
%\newcommand{ \vphiDL }[1]{ \varphi_{\mathrm{DL}}( #1 ) }
%\newcommand{ \vphiCDL }[1]{ \varphi_{\mathrm{CDL}}( #1 ) }
%\newcommand{ \TvphiCDL }[1]{ \ol{\varphi}_{\mathrm{CDL}}( #1 ) }
%\newcommand{ \HvphiCDL }[1]{ \wh{\varphi}_{\mathrm{CDL}}( #1 ) }
%\newcommand{ \vphiICA }[1]{ \varphi_{\mathrm{ICA}}( #1 ) }

\newcommand{ \init }[1]{{\mathbf #1}_{\mathrm{init}}}

\newcommand{\qq}[1]{{\color{blue}{\bf Qing: #1}}}
\newcommand{\xiao}[1]{{\color{magenta}{\bf Xiao: #1}}}
\newcommand{\sz}[1]{{\color{blue}{\bf Simon: #1}}}
\newcommand{\zz}[1]{{\color{blue}{\bf Zhihui: #1}}}
\newcommand{\zzedit}[1]{{\color{purple}{#1}}}
\newcommand{\cy}[1]{{\color{blue}{\bf Chong: #1}}}
\newcommand{\td}[1]{{\color{magenta}{\bf TODO: #1}}}
\newcommand{\jz}[1]{{\color{magenta}{\bf Jinxin: #1}}}
%\newcommand{\edit}[1]{{\color{black}{#1}}}
\newcommand{\edited}[1]{{\color{black}{#1}}}

%\numberwithin{equation}{section}

\def \endprf{\hfill {\vrule height6pt width6pt depth0pt}\medskip}
\newenvironment{proof}{\noindent {\bf Proof} }{\endprf\par}

\newcommand{\qed}{{\unskip\nobreak\hfil\penalty50\hskip2em\vadjust{}
           \nobreak\hfil$\Box$\parfillskip=0pt\finalhyphendemerits=0\par}}


\newcommand{\mr}{\mathrm}
\newcommand{\inprod}[2]{\langle#1,#2\rangle}
%\newcommand{\parans}[1]{\left(#1\right)}


\newcommand{\res}[2]{\mb \iota_{ #1 \rightarrow #2  }}
\newcommand{\shift}[2]{{\mathrm{s}_{#2}}\left[#1\right]}
\newcommand{\Shift}[2]{{\wh{\mathrm{s}}_{#2}}\left[#1\right]}

==> NeurIPS_2022/qq_defs.tex <==


%\usepackage{tgpagella}
%\usepackage[utf8]{inputenc} % allow utf-8 input
%\usepackage[T1]{fontenc}    % use 8-bit T1 fonts

\usepackage{url}
%\usepackage{hyperref}       % hyperlinks
%\usepackage{url}            % simple URL typesetting
%\usepackage{booktabs}       % professional-quality tables
%\usepackage{nicefrac}       % compact symbols for 1/2, etc.
%\usepackage{microtype}      % microtypography
%\usepackage{authblk}
%\usepackage{multirow}
%\usepackage{mathabx}

%\usepackage{graphicx,amsmath,amsfonts,amscd,amssymb,bm,url,color,latexsym}
%\usepackage[margin=0.95in]{geometry}

%\usepackage[inline]{enumitem}
%\usepackage{mwe}
%\usepackage{subfigure}
%\usepackage{subfig}
%\usepackage{subcaption}
%\usepackage{bbm}
%\usepackage{bm}
%\usepackage{microtype}
%\setlength{\captionmargin}{30pt}
%\usepackage{algorithm,algorithmicx}
%\usepackage{algpseudocode}
%\usepackage{hyperref}
%\usepackage[nameinlink]{cleveref}
%\usepackage{verbatim}
%\usepackage{framed}
%\usepackage{comment}
%\usepackage{wrapfig}
%\usepackage{tikz}
%\usepackage{pgfplots}

%\usepackage{cite}
%\usepackage{tikz}
%\usepackage{multirow}
%\usepackage{cleveref}

%\usepackage{tablefootnote}
%\usepackage{tcolorbox}
%\usepackage{pifont}
%\usepackage{authblk}
%\usepackage[margin=0.95in]{geometry}

\providecommand{\keywords}[1]{\textbf{\textit{Index terms---}} #1}


% pagebreak for long equations
%\allowdisplaybreaks

\hypersetup{
    colorlinks=true,%
    citecolor=blue,%
    filecolor=blue,%
    linkcolor=blue,%
    urlcolor=blue
}
\usepackage[toc, page]{appendix}
%%%%%%%%%%%%%%
\renewcommand\floatpagefraction{.95}
\renewcommand\topfraction{.95}
\renewcommand\bottomfraction{.95}
\renewcommand\textfraction{.05}
\setcounter{totalnumber}{50}
\setcounter{topnumber}{50}
\setcounter{bottomnumber}{50}
%%%%%%%%%%%%%%
%--------------
\newtheorem{theorem}{Theorem}[section]
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{proposition}[theorem]{Proposition}
%\newtheorem{definition}[theorem]{Definition}
\newtheorem{definition}{Definition}
\newtheorem{conjecture}[theorem]{Conjecture}
%\newtheorem{problem}[theorem]{Problem}
%\newtheorem{claim}[theorem]{Claim}
\newtheorem{remark}[theorem]{Remark}
%\newtheorem{example}[theorem]{Example}
%\newtheorem{assumption}[theorem]{Assumption}


\newcommand{\indep}{\rotatebox[origin=c]{90}{$\models$}}

\renewcommand{\mathbf}{\boldsymbol}

%\newcommand{\conv}{\circledast}
\newcommand{\cconv}{  \boxasterisk }
%\newcommand{\mb}{\mathbf}
%\newcommand{\mc}{\mathcal}
%\newcommand{\mf}{\mathfrak}
\newcommand{\md}{\mathds}
%\newcommand{\bb}{\mathbb}
\newcommand{\magnitude}[1]{ \left| #1 \right| }
%\newcommand{\set}[1]{\left\{ #1 \right\}}
\newcommand{\condset}[2]{ \left\{ #1 \;\middle|\; #2 \right\} }



%\newcommand{\reals}{\bb R}
\newcommand{\proj}{\mathrm{proj}}
%\newcommand{\E}{\mathbb{E}}

%\newcommand{\eps}{\varepsilon}
%\newcommand{\R}{\reals}
\newcommand{\Cp}{\bb C}
%\newcommand{\Z}{\bb Z}
%\newcommand{\N}{\bb N}
\newcommand{\Sp}{\bb S}
\newcommand{\Ba}{\bb B}
\newcommand{\indicator}[1]{\mathbbm 1_{#1}}
\renewcommand{\P}{\mathbb{P}}

\newcommand{ \Brac }[1]{\left\lbrace #1 \right\rbrace}
\newcommand{ \brac }[1]{\left[ #1 \right]}
\newcommand{ \paren }[1]{ \left( #1 \right) }
\newcommand{\col}{\mathrm{col}}


\newcommand{\Lce}{\mc L_{\mathrm{CE}}}

% to declare new operator
% \DeclareMathOperator{\xxx}{xxx}
%\DeclareMathOperator{\dist}{dist}
\DeclareMathOperator{\poly}{poly}
%\DeclareMathOperator{\rank}{rank}
%\DeclareMathOperator{\trace}{tr}
\DeclareMathOperator{\supp}{supp}
\DeclareMathOperator{\vect}{vec}
%\DeclareMathOperator{\diag}{diag}
%\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\grad}{grad}
\DeclareMathOperator{\Hess}{Hess}
\DeclareMathOperator{\mini}{minimize}
\DeclareMathOperator{\maxi}{maximize}
%\DeclareMathOperator{\st}{subject\; to}

%% Other definitions


%\newcommand{\wh}{\widehat}
%\newcommand{\wt}{\widetilde}
%\newcommand{\ol}{\overline}
%\newcommand{\wc}{\widecheck}



%\newcommand{\norm}[2]{\left\| #1 \right\|_{#2}}
%\newcommand{\abs}[1]{\left| #1 \right|}
%\newcommand{\innerprod}[2]{\left\langle #1,  #2 \right\rangle}
%\newcommand{\prob}[1]{\bb P\left[ #1 \right]}
%\newcommand{\expect}[1]{\bb E\left[ #1 \right]}
%\newcommand{\function}[2]{#1 \left(#2\right)}
%\newcommand{\integral}[4]{\int_{#1}^{#2}\; #3\; #4}


%\newcommand{ \vphi }[1]{ \varphi( #1 ) }
%\newcommand{ \vphiT }[1]{ \varphi_{\mathrm{T}}( #1 ) }
%\newcommand{ \vphiDL }[1]{ \varphi_{\mathrm{DL}}( #1 ) }
%\newcommand{ \vphiCDL }[1]{ \varphi_{\mathrm{CDL}}( #1 ) }
%\newcommand{ \TvphiCDL }[1]{ \ol{\varphi}_{\mathrm{CDL}}( #1 ) }
%\newcommand{ \HvphiCDL }[1]{ \wh{\varphi}_{\mathrm{CDL}}( #1 ) }
%\newcommand{ \vphiICA }[1]{ \varphi_{\mathrm{ICA}}( #1 ) }

\newcommand{ \init }[1]{{\mathbf #1}_{\mathrm{init}}}

\newcommand{\qq}[1]{{\color{blue}{\bf Qing: #1}}}
\newcommand{\xiao}[1]{{\color{magenta}{\bf Xiao: #1}}}
\newcommand{\sz}[1]{{\color{blue}{\bf Simon: #1}}}
\newcommand{\zz}[1]{{\color{blue}{\bf Zhihui: #1}}}
\newcommand{\zzedit}[1]{{\color{purple}{#1}}}
\newcommand{\cy}[1]{{\color{blue}{\bf Chong: #1}}}
\newcommand{\td}[1]{{\color{magenta}{\bf TODO: #1}}}
\newcommand{\jz}[1]{{\color{magenta}{\bf Jinxin: #1}}}
%\newcommand{\edit}[1]{{\color{black}{#1}}}
\newcommand{\edited}[1]{{\color{black}{#1}}}

%\numberwithin{equation}{section}

\def \endprf{\hfill {\vrule height6pt width6pt depth0pt}\medskip}
\newenvironment{proof}{\noindent {\bf Proof} }{\endprf\par}

\newcommand{\qed}{{\unskip\nobreak\hfil\penalty50\hskip2em\vadjust{}
           \nobreak\hfil$\Box$\parfillskip=0pt\finalhyphendemerits=0\par}}


\newcommand{\mr}{\mathrm}
\newcommand{\inprod}[2]{\langle#1,#2\rangle}
%\newcommand{\parans}[1]{\left(#1\right)}


\newcommand{\res}[2]{\mb \iota_{ #1 \rightarrow #2  }}
\newcommand{\shift}[2]{{\mathrm{s}_{#2}}\left[#1\right]}
\newcommand{\Shift}[2]{{\wh{\mathrm{s}}_{#2}}\left[#1\right]}

==> macro.tex <==



\usepackage{amsmath,amssymb,amsbsy,amsfonts,amscd,bm,url,color,latexsym}
\usepackage[hidelinks]{hyperref}
%amsthm, graphicx,amsmath,,amssymb,
\usepackage{paralist}
\usepackage[dvipsnames]{xcolor}
\usepackage{color}
\usepackage{graphicx}
\graphicspath{{./figs/}}
\usepackage{algorithm}
\usepackage{algorithmic}
\usepackage{comment}
\usepackage{multirow}
\usepackage{enumitem}
\usepackage{fancyhdr}
\usepackage{cite}
%\usepackage{citesort}
\usepackage{cleveref}
\usepackage{subcaption}
\usepackage{authblk}
% Theorems
%\def \remarks {\noindent {\bf Remarks.}\ \ }
\newtheorem{thm}{Theorem}%[section] %(If you want theorem numbered
%\newtheorem{lemma}{Lemma}%[section] %%    with section number.
\newtheorem{cor}{Corollary}%[section]
\newtheorem{prop}{Proposition}%[section]
%\newtheorem{definition}{Definition}%[section]
\newtheorem{defi}{Definition}%[section]
\newtheorem{assum}{Assumption}
%\newtheorem*{goal}{Plan}
%\newtheorem{theorem}{Theorem}
\newtheorem{lem}{Lemma}
%\theoremstyle{remark}
%\newtheorem{remark}{Remark}
%\theoremstyle{problem}
%\newtheorem{problem}{Problem}

% fields
\renewcommand{\O}{\mathbb{O}}
\newcommand{\R}{\mathbb{R}}
\def \real    { \mathbb{R} }
\def \reals   { \mathbb{R} }
\def \Real {\mathbb{R}}
\newcommand{\C}{\mathbb{C}}
\def \complex{\mathbb{C}}
\def \Complex {\mathbb{C}}
\newcommand{\Z}{\mathbb{Z}}
\newcommand{\N}{\mathbb{N}}

\newcommand{\la}{\left\langle}
\newcommand{\ra}{\right\rangle}
\newcommand{\e}{\begin{equation}}
\newcommand{\ee}{\end{equation}}
\newcommand{\en}{\begin{equation*}}
\newcommand{\een}{\end{equation*}}
\newcommand{\eqn}{\begin{eqnarray}}
\newcommand{\eeqn}{\end{eqnarray}}
\newcommand{\bmat}{\begin{bmatrix}}
\newcommand{\emat}{\end{bmatrix}}
% complex numbers
\renewcommand{\Re}[1]{\operatorname{Re}\left\{#1\right\}}
\renewcommand{\Im}[1]{\operatorname{Im}\left\{#1\right\}}
\newcommand{\conj}[1]{\mkern 1.5mu\overline{\mkern-1.5mu#1\mkern-1.5mu}\mkern 1.5mu}

\DeclareMathAlphabet\mathbfcal{OMS}{cmsy}{b}{n}
% probability and stat
\renewcommand{\P}[1]{\operatorname{\mathbb{P}}\left(#1\right)}
\newcommand{\E}{\operatorname{\mathbb{E}}}
\newcommand{\dif}{\operatorname{d}}
\newcommand{\var}{\operatorname{var}}

% calculus
\renewcommand{\d}[1]{\,\mathrm{d}#1}

% constants (written in roman, if wanted)
%\newcommand{\e}{\mathrm{e}}
\renewcommand{\j}{\mathrm{j}}




\newcommand{\mb}{\mathbf}
\newcommand{\mc}{\mathcal}
\newcommand{\mf}{\mathfrak}
\newcommand{\bb}{\mathbb}
\newcommand{\mrm}{\mathrm}
\newcommand{\mtt}{\mathtt}
\def \vecword  {\operatorname*{vec}}
% linear algebra
% 	vector notation
\newcommand{\vct}[1]{\boldsymbol{#1}}
%   matrices
\newcommand{\mtx}[1]{\boldsymbol{#1}}
%   block vector
\newcommand{\bvct}[1]{\mathbf{#1}}
%   block matrix
\newcommand{\bmtx}[1]{\mathbf{#1}}
%	inner products
\newcommand{\inner}[1]{\left<#1\right>}
\newcommand{\<}{\langle}
\renewcommand{\>}{\rangle}
% 	transpose, Hermitian, pseudo-inverse
\renewcommand{\H}{\mathrm{H}}
\newcommand{\T}{\mathrm{T}}
\newcommand{\pinv}{\dagger}
%	fundamental subspaces
\newcommand{\Null}{\operatorname{Null}}
\newcommand{\Range}{\operatorname{Range}}
\newcommand{\Span}{\operatorname{Span}}
%	operators
\newcommand{\trace}{\operatorname{trace}}
\newcommand{\conv}{\operatorname{conv}}
\newcommand{\rank}{\operatorname{rank}}
\newcommand{\diag}{\operatorname{diag}}
\newcommand{\toep}{\operatorname{Toep}}
\newcommand{\SDP}{\operatorname{SDP}}
\newcommand{\PSD}{\operatorname{PSD}}
\newcommand{\far}{\operatorname{far}}
\newcommand{\near}{\operatorname{near}}
\newcommand{\sign}{\operatorname{sign}}
\newcommand{\sgn}{\operatorname{sgn}}
\newcommand{\Sign}{\operatorname{Sgn}}
\newcommand{\dist}{\operatorname{dist}}
\def \lg        {\langle}
\def \rg        {\rangle}
\def \vec       {\operatorname*{vec}}
%
\newcommand{\dimension}{\operatorname{dim}}

% sets and topology
\newcommand{\set}[1]{\mathbb{#1}}
\newcommand{\closure}{\operatorname{cl}}	% closure
\newcommand{\interior}{\operatorname{int}}
\newcommand{\boundary}{\operatorname{bd}}
\newcommand{\diameter}{\operatorname{diam}}

% functional analysis
\newcommand{\domain}{\operatorname{dom}}
\newcommand{\epigraph}{\operatorname{epi}}
\newcommand{\hypograph}{\operatorname{hypo}}
\newcommand{\linop}[1]{\mathscr{#1}}	% general linear operator

% optimization
\DeclareMathOperator*{\minimize}{\text{minimize}}
\DeclareMathOperator*{\maximize}{\text{maximize}}
\DeclareMathOperator*{\argmin}{\text{arg~min}}
\DeclareMathOperator*{\argmax}{\text{arg~max}}
\def \st {\operatorname*{s.t.\ }}
% other
%\newcommand{\sgn}{\text{sgn}}
\newcommand{\sinc}{\text{sinc}}
\newcommand{\floor}[1]{\left\lfloor #1 \right\rfloor}
\newcommand{\ceil}[1]{\left\lceil #1 \right\rceil}
\newcommand{\eps}{\epsilon}


\newcommand{\wh}{\widehat}
\newcommand{\wc}{\widecheck}
\newcommand{\wt}{\widetilde}
\newcommand{\ol}{\overline}
\newcommand{\NC}{$\mc {NC}$}

\newcommand{\norm}[2]{\left\| #1 \right\|_{#2}}
\newcommand{\nrm}[1]{\left\Vert#1\right\Vert}
\newcommand{\abs}[1]{\left| #1 \right|}
\newcommand{\bracket}[1]{\left( #1 \right)}
\newcommand{\parans}[1]{\left(#1\right)}
\newcommand{\innerprod}[2]{\left\langle #1,  #2 \right\rangle}
\newcommand{\prob}[1]{\bb P\left[ #1 \right]}
\newcommand{\expect}[1]{\bb E\left[ #1 \right]}
\newcommand{\function}[2]{#1 \left(#2\right)}
\newcommand{\integral}[4]{\int_{#1}^{#2}\; #3\; #4}
\newcommand{\iter}[1]{^{(#1)}}
\newcommand*\samethanks[1][\value{footnote}]{\footnotemark[#1]}

\newcommand{\js}[1]{{\color{blue} [\noindent JS: #1]}}

%--------------------------------------------------------------------------
\newcommand{\calA}{\mathcal{A}}
\newcommand{\calB}{\mathcal{B}}
\newcommand{\calC}{\mathcal{C}}
\newcommand{\calD}{\mathcal{D}}
\newcommand{\calE}{\mathcal{E}}
\newcommand{\calF}{\mathcal{F}}
\newcommand{\calG}{\mathcal{G}}
\newcommand{\calH}{\mathcal{H}}
\newcommand{\calI}{\mathcal{I}}
\newcommand{\calJ}{\mathcal{J}}
\newcommand{\calK}{\mathcal{K}}
\newcommand{\calL}{\mathcal{L}}
\newcommand{\calM}{\mathcal{M}}
\newcommand{\calN}{\mathcal{N}}
\newcommand{\calO}{\mathcal{O}}
\newcommand{\calP}{\mathcal{P}}
\newcommand{\calQ}{\mathcal{Q}}
\newcommand{\calR}{\mathcal{R}}
\newcommand{\calS}{\mathcal{S}}
\newcommand{\calT}{\mathcal{T}}
\newcommand{\calU}{\mathcal{U}}
\newcommand{\calV}{\mathcal{V}}
\newcommand{\calW}{\mathcal{W}}
\newcommand{\calX}{\mathcal{X}}
\newcommand{\calY}{\mathcal{Y}}
\newcommand{\calZ}{\mathcal{Z}}





\newcommand{\va}{\vct{a}}
\newcommand{\vb}{\vct{b}}
\newcommand{\vc}{\vct{c}}
\newcommand{\vd}{\vct{d}}
\newcommand{\ve}{\vct{e}}
\newcommand{\vf}{\vct{f}}
\newcommand{\vg}{\vct{g}}
\newcommand{\vh}{\vct{h}}
\newcommand{\vi}{\vct{i}}
\newcommand{\vj}{\vct{j}}
\newcommand{\vk}{\vct{k}}
\newcommand{\vl}{\vct{l}}
\newcommand{\vm}{\vct{m}}
\newcommand{\vn}{\vct{n}}
\newcommand{\vo}{\vct{o}}
\newcommand{\vp}{\vct{p}}
\newcommand{\vq}{\vct{q}}
\newcommand{\vr}{\vct{r}}
\newcommand{\vs}{\vct{s}}
\newcommand{\vt}{\vct{t}}
\newcommand{\vu}{\vct{u}}
\newcommand{\vv}{\vct{v}}
\newcommand{\vw}{\vct{w}}
\newcommand{\vx}{\vct{x}}
\newcommand{\vy}{\vct{y}}
\newcommand{\vz}{\vct{z}}
%
\newcommand{\valpha}{\vct{\alpha}}
\newcommand{\vbeta}{\vct{\beta}}
\newcommand{\vtheta}{\vct{\theta}}
\newcommand{\vepsilon}{\vct{\epsilon}}
\newcommand{\veps}{\vct{\epsilon}}
\newcommand{\vvarepsilon}{\vct{\varepsilon}}
\newcommand{\vgamma}{\vct{\gamma}}
\newcommand{\vlambda}{\vct{\lambda}}
\newcommand{\vnu}{\vct{\nu}}
\newcommand{\vphi}{\vct{\phi}}
\newcommand{\vpsi}{\vct{\psi}}
\newcommand{\vdelta}{\vct{\delta}}
\newcommand{\veta}{\vct{\eta}}
\newcommand{\vxi}{\vct{\xi}}
\newcommand{\vmu}{\vct{\mu}}
\newcommand{\vrho}{\vct{\rho}}
%
\newcommand{\vzero}{\vct{0}}
\newcommand{\vone}{\vct{1}}


\newcommand{\mA}{\mtx{A}}
\newcommand{\mB}{\mtx{B}}
\newcommand{\mC}{\mtx{C}}
\newcommand{\mD}{\mtx{D}}
\newcommand{\mE}{\mtx{E}}
\newcommand{\mF}{\mtx{F}}
\newcommand{\mG}{\mtx{G}}
\newcommand{\mH}{\mtx{H}}
\newcommand{\mJ}{\mtx{J}}
\newcommand{\mK}{\mtx{K}}
\newcommand{\mL}{\mtx{L}}
\newcommand{\mM}{\mtx{M}}
\newcommand{\mN}{\mtx{N}}
\newcommand{\mO}{\mtx{O}}
\newcommand{\mP}{\mtx{P}}
\newcommand{\mQ}{\mtx{Q}}
\newcommand{\mR}{\mtx{R}}
\newcommand{\mS}{\mtx{S}}
\newcommand{\mT}{\mtx{T}}
\newcommand{\mU}{\mtx{U}}
\newcommand{\mV}{\mtx{V}}
\newcommand{\mW}{\mtx{W}}
\newcommand{\mX}{\mtx{X}}
\newcommand{\mY}{\mtx{Y}}
\newcommand{\mZ}{\mtx{Z}}
%
\newcommand{\mGamma}{\mtx{\Gamma}}
\newcommand{\mDelta}{\mtx{\Delta}}
\newcommand{\mLambda}{\mtx{\Lambda}}
\newcommand{\mOmega}{\mtx{\Omega}}
\newcommand{\mPhi}{\mtx{\Phi}}
\newcommand{\mPsi}{\mtx{\Psi}}
\newcommand{\mSigma}{\mtx{\Sigma}}
\newcommand{\mTheta}{\mtx{\Theta}}
\newcommand{\mUpsilon}{\mtx{\Upsilon}}
%
\newcommand{\mId}{\bmtx{I}}
\newcommand{\mEx}{{\bf J}}
\newcommand{\mzero}{{\bf 0}}
\newcommand{\mone}{{\bf 1}}
%
\newcommand{\bva}{\bvct{a}}
\newcommand{\bvh}{\bvct{h}}
\newcommand{\bvw}{\bvct{w}}
\newcommand{\bvx}{\bvct{x}}
\newcommand{\bvy}{\bvct{y}}


\newcommand{\bmM}{\bmtx{M}}
\newcommand{\bmH}{\bmtx{H}}
\newcommand{\bmX}{\bmtx{X}}


\newcommand{\setA}{\set{A}}
\newcommand{\setB}{\set{B}}
\newcommand{\setC}{\set{C}}
\newcommand{\setD}{\set{D}}
\newcommand{\setE}{\set{E}}
\newcommand{\setF}{\set{F}}
\newcommand{\setG}{\set{G}}
\newcommand{\setH}{\set{H}}
\newcommand{\setI}{\set{I}}
\newcommand{\setJ}{\set{J}}
\newcommand{\setK}{\set{K}}
\newcommand{\setL}{\set{L}}
\newcommand{\setM}{\set{M}}
\newcommand{\setN}{\set{N}}
\newcommand{\setO}{\set{O}}
\newcommand{\setP}{\set{P}}
\newcommand{\setQ}{\set{Q}}
\newcommand{\setR}{\set{R}}
\newcommand{\setS}{\set{S}}
\newcommand{\setT}{\set{T}}
\newcommand{\setU}{\set{U}}
\newcommand{\setV}{\set{V}}
\newcommand{\setW}{\set{W}}
\newcommand{\setX}{\set{X}}
\newcommand{\setY}{\set{Y}}
\newcommand{\setZ}{\set{Z}}

\renewcommand{\ss}{{\vspace*{-1mm}}}

\setcounter{MaxMatrixCols}{20}

%\pagestyle{plain}

\graphicspath{{./figs/}}

\newlength{\imgwidth}
\setlength{\imgwidth}{3.125in}

\newcommand{\QW}[1]{\textcolor{red}{\bf [{\em QW:} #1]}}
\newcommand{\note}[1]{\textcolor{blue}{\bf [{\em Note:} #1]}}
\newcommand{\revise}[1]{\textcolor{black}{#1}}
\newcommand{\edit}[1]{\textcolor{red}{#1}}

\newboolean{twoColVersion}
\setboolean{twoColVersion}{false}
\newcommand{\twoCol}[2]{\ifthenelse{\boolean{twoColVersion}} {#1} {#2} }


\newcommand{\Poff}{\mathcal{P}_{\textup{off}}}
\newcommand{\Pon}{\mathcal{P}_{\textup{diag}}}

\usepackage{tikz}
\usepackage{tikz-3dplot}
\usepackage{pgfplots}
\usepgfplotslibrary{patchplots}
\usetikzlibrary{patterns, positioning, arrows}
\pgfplotsset{compat=1.15}



==> qq_defs.tex <==


% \usepackage{tgpagella}
% \usepackage[utf8]{inputenc} % allow utf-8 input
% \usepackage[T1]{fontenc}    % use 8-bit T1 fonts
% \usepackage{url}
%\usepackage{hyperref}       % hyperlinks
%\usepackage{url}            % simple URL typesetting
%\usepackage{booktabs}       % professional-quality tables
%\usepackage{nicefrac}       % compact symbols for 1/2, etc.
%\usepackage{microtype}      % microtypography
%\usepackage{authblk}
%\usepackage{multirow}
%\usepackage{mathabx}

%\usepackage{graphicx,amsmath,amsfonts,amscd,amssymb,bm,url,color,latexsym}
%\usepackage[margin=0.95in]{geometry}

%\usepackage[inline]{enumitem}
%\usepackage{mwe}
%\usepackage{subfigure}
%\usepackage{subfig}
%\usepackage{subcaption}
%\usepackage{bbm}
%\usepackage{bm}
%\usepackage{microtype}
%\setlength{\captionmargin}{30pt}
%\usepackage{algorithm,algorithmicx}
%\usepackage{algpseudocode}
%\usepackage{hyperref}
%\usepackage[nameinlink]{cleveref}
%\usepackage{verbatim}
%\usepackage{framed}
%\usepackage{comment}
%\usepackage{wrapfig}
%\usepackage{tikz}
%\usepackage{pgfplots}

%\usepackage{cite}
%\usepackage{tikz}
%\usepackage{multirow}
%\usepackage{cleveref}

%\usepackage{tablefootnote}
%\usepackage{tcolorbox}
%\usepackage{pifont}
%\usepackage{authblk}
%\usepackage[margin=0.95in]{geometry}

% \providecommand{\keywords}[1]{\textbf{\textit{Index terms---}} #1}


% pagebreak for long equations
%\allowdisplaybreaks

% \hypersetup{
%     colorlinks=true,%
%     citecolor=blue,%
%     filecolor=blue,%
%     linkcolor=blue,%
%     urlcolor=blue
% }
% \usepackage[toc, page]{appendix}
%%%%%%%%%%%%%%
% \renewcommand\floatpagefraction{.95}
% \renewcommand\topfraction{.95}
% \renewcommand\bottomfraction{.95}
% \renewcommand\textfraction{.05}
% \setcounter{totalnumber}{50}
% \setcounter{topnumber}{50}
% \setcounter{bottomnumber}{50}
%%%%%%%%%%%%%%
%--------------
% \newtheorem{theorem}{Theorem}[section]
% \newtheorem{lemma}[theorem]{Lemma}
% \newtheorem{corollary}[theorem]{Corollary}
% \newtheorem{proposition}[theorem]{Proposition}
% \newtheorem{definition}[theorem]{Definition}
% \newtheorem{conjecture}[theorem]{Conjecture}
%\newtheorem{problem}[theorem]{Problem}
%\newtheorem{claim}[theorem]{Claim}
% \newtheorem{remark}[theorem]{Remark}
%\newtheorem{example}[theorem]{Example}
%\newtheorem{assumption}[theorem]{Assumption}


\newcommand{\indep}{\rotatebox[origin=c]{90}{$\models$}}

\renewcommand{\mathbf}{\boldsymbol}

%\newcommand{\conv}{\circledast}
\newcommand{\cconv}{  \boxasterisk }
%\newcommand{\mb}{\mathbf}
%\newcommand{\mc}{\mathcal}
%\newcommand{\mf}{\mathfrak}
\newcommand{\md}{\mathds}
%\newcommand{\bb}{\mathbb}
\newcommand{\magnitude}[1]{ \left| #1 \right| }
%\newcommand{\set}[1]{\left\{ #1 \right\}}
\newcommand{\condset}[2]{ \left\{ #1 \;\middle|\; #2 \right\} }



%\newcommand{\reals}{\bb R}
\newcommand{\proj}{\mathrm{proj}}
%\newcommand{\E}{\mathbb{E}}

%\newcommand{\eps}{\varepsilon}
%\newcommand{\R}{\reals}
\newcommand{\Cp}{\bb C}
%\newcommand{\Z}{\bb Z}
%\newcommand{\N}{\bb N}
\newcommand{\Sp}{\bb S}
\newcommand{\Ba}{\bb B}
\newcommand{\indicator}[1]{\mathbbm 1_{#1}}
\renewcommand{\P}{\mathbb{P}}

\newcommand{ \Brac }[1]{\left\lbrace #1 \right\rbrace}
\newcommand{ \brac }[1]{\left[ #1 \right]}
\newcommand{ \paren }[1]{ \left( #1 \right) }
\newcommand{\col}{\mathrm{col}}

\newcommand{\Lce}{\mc L_{\mathrm{CE}}}
\newcommand{\Lls}{\mc L_{\mathrm{LS}}}
\newcommand{\Lfl}{\mc L_{\mathrm{FL}}}
\newcommand{\Lmse}{\mc L_{\mathrm{LMSE}}}

% % to declare new operator
% % \DeclareMathOperator{\xxx}{xxx}
% %\DeclareMathOperator{\dist}{dist}
% \DeclareMathOperator{\poly}{poly}
% %\DeclareMathOperator{\rank}{rank}
% %\DeclareMathOperator{\trace}{tr}
% \DeclareMathOperator{\supp}{supp}
% \DeclareMathOperator{\vect}{vec}
% %\DeclareMathOperator{\diag}{diag}
% %\DeclareMathOperator{\sign}{sign}
% \DeclareMathOperator{\grad}{grad}
% \DeclareMathOperator{\Hess}{Hess}
% \DeclareMathOperator{\mini}{minimize}
% \DeclareMathOperator{\maxi}{maximize}
%\DeclareMathOperator{\st}{subject\; to}

%% Other definitions


%\newcommand{\wh}{\widehat}
%\newcommand{\wt}{\widetilde}
%\newcommand{\ol}{\overline}
%\newcommand{\wc}{\widecheck}



%\newcommand{\norm}[2]{\left\| #1 \right\|_{#2}}
%\newcommand{\abs}[1]{\left| #1 \right|}
%\newcommand{\innerprod}[2]{\left\langle #1,  #2 \right\rangle}
%\newcommand{\prob}[1]{\bb P\left[ #1 \right]}
%\newcommand{\expect}[1]{\bb E\left[ #1 \right]}
%\newcommand{\function}[2]{#1 \left(#2\right)}
%\newcommand{\integral}[4]{\int_{#1}^{#2}\; #3\; #4}


%\newcommand{ \vphi }[1]{ \varphi( #1 ) }
%\newcommand{ \vphiT }[1]{ \varphi_{\mathrm{T}}( #1 ) }
%\newcommand{ \vphiDL }[1]{ \varphi_{\mathrm{DL}}( #1 ) }
%\newcommand{ \vphiCDL }[1]{ \varphi_{\mathrm{CDL}}( #1 ) }
%\newcommand{ \TvphiCDL }[1]{ \ol{\varphi}_{\mathrm{CDL}}( #1 ) }
%\newcommand{ \HvphiCDL }[1]{ \wh{\varphi}_{\mathrm{CDL}}( #1 ) }
%\newcommand{ \vphiICA }[1]{ \varphi_{\mathrm{ICA}}( #1 ) }

\newcommand{ \init }[1]{{\mathbf #1}_{\mathrm{init}}}

\newcommand{\qq}[1]{{\color{blue}{\bf Qing: #1}}}
\newcommand{\xiao}[1]{{\color{magenta}{\bf Xiao: #1}}}
\newcommand{\sz}[1]{{\color{blue}{\bf Simon: #1}}}
\newcommand{\zz}[1]{{\color{blue}{{\bf Zhihui:} #1}}}
\newcommand{\zzedit}[1]{{\color{purple}{#1}}}
\newcommand{\cy}[1]{{\color{blue}{\bf Chong: #1}}}
\newcommand{\td}[1]{{\color{magenta}{\bf TODO: #1}}}
\newcommand{\jz}[1]{{\color{magenta}{\bf Jinxin: #1}}}
%\newcommand{\edit}[1]{{\color{black}{#1}}}
\newcommand{\edited}[1]{{\color{black}{#1}}}

%\numberwithin{equation}{section}

\def \endprf{\hfill {\vrule height6pt width6pt depth0pt}\medskip}
\newenvironment{proof}{\noindent {\bf Proof} }{\endprf\par}

\newcommand{\qed}{{\unskip\nobreak\hfil\penalty50\hskip2em\vadjust{}
           \nobreak\hfil$\Box$\parfillskip=0pt\finalhyphendemerits=0\par}}


\newcommand{\mr}{\mathrm}
\newcommand{\inprod}[2]{\langle#1,#2\rangle}
%\newcommand{\parans}[1]{\left(#1\right)}


\newcommand{\res}[2]{\mb \iota_{ #1 \rightarrow #2  }}
\newcommand{\shift}[2]{{\mathrm{s}_{#2}}\left[#1\right]}
\newcommand{\Shift}[2]{{\wh{\mathrm{s}}_{#2}}\left[#1\right]}
